ARise: Towards Knowledge-Augmented Reasoning via Risk-Adaptive Search

Large language models (LLMs) have demonstrated impressive capabilities and are receiving increasing attention to enhance their reasoning through scaling test--time compute. However, their application in open--ended, knowledge--intensive, complex reasoning scenarios is still limited. Reasoning--oriented methods struggle to generalize to open--ended scenarios due to implicit assumptions of complete world knowledge. Meanwhile, knowledge--augmented reasoning (KAR) methods fail to address two core challenges: 1) error propagation, where errors in early steps cascade through the chain, and 2) verification bottleneck, where the explore--exploit tradeoff arises in multi--branch decision processes. To overcome these limitations, we introduce ARise, a novel framework that integrates risk assessment of intermediate reasoning states with dynamic retrieval--augmented generation (RAG) within a Monte Carlo tree search paradigm. This approach enables effective construction and optimization of reasoning plans across multiple maintained hypothesis branches. Experimental results show that ARise significantly outperforms the state--of--the--art KAR methods by up to 23.10%, and the latest RAG-equipped large reasoning models by up to 25.37%. Our project page is at https://opencausalab.github.io/ARise.

==> Tables/algorithm.tex <==
% 算法表
\begin{table*}[t]
\centering
\begin{tabular}{>{\quad}l>{\raggedleft\arraybackslash}p{7.5cm}} % 第二列右对齐
\toprule
\multicolumn{2}{l}{\textbf{Algorithm 1} \sys} \\
\midrule
\multicolumn{2}{l}{\textbf{Require:} original problem $q$; prompt $p_d$ for decomposition; prompt $p_r$ for reasoning} \\
\multicolumn{2}{l}{\textbf{Require:} LLM $f(\cdot)$; external knowledge retrieval model $g(\cdot)$} \\
\multicolumn{2}{l}{\textbf{Require:} selecte $Se(\cdot)$; expand $Ex(\cdot)$; simulate $Si(\cdot)$; back-propagate $Ba(\cdot)$} \\
\multicolumn{2}{l}{\textbf{Require:} prompt $p_g$ for problem generation; value function $V(\cdot)$; get best path $P(\cdot)$} \\
$\mathbf{s_0}; \mathbf{t} \leftarrow q$                     & $\triangleright$ Generate root node and tree \\
\textbf{for} $i=1,\dots,T$ \textbf{do}                      & $\triangleright$ Perform T MCTS iterations   \\
\quad $\mathbf{s_i} \leftarrow Se(\mathbf{s_0}, \mathbf{t})$     & $\triangleright$ Select the best node        \\
\quad $d_i \leftarrow f(\mathbf{s_i}, q, p_d)$                    & $\triangleright$ Decompose the problem       \\
\quad $z_i \leftarrow g(d_i)$                                     & $\triangleright$ Retrieve relevant documents  \\
\quad $r_i \leftarrow f(z_i, d_i, p_r)$                           & $\triangleright$ Reason forward               \\
\quad $\mathbf{s_{i+1}} \leftarrow \mathbf{s_i}, r_i, V(f(r_i, q, p_g))$ & $\triangleright$ Generate new nodes \\
\quad $\mathbf{t} \leftarrow Ex(\mathbf{s_{i+1}})$               & $\triangleright$ Append nodes to the tree     \\
\quad $\mathbf{t} \leftarrow Si(\mathbf{s_i})$; $Ba(\mathbf{s_i}, \mathbf{s_0})$ & $\triangleright$ Simulate and Back-propagate  \\
\textbf{end for}                                            &                                               \\
\textbf{return} $P(\mathbf{s_0}, \mathbf{t})$               & $\triangleright$ Get best path                \\
\bottomrule
\end{tabular}
\label{tab:algorithm}
\end{table*}

==> Tables/overhead.tex <==
\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{>{\centering\arraybackslash}p{2.2cm}
                >{\centering\arraybackslash}p{1.2cm}
                >{\centering\arraybackslash}p{1.2cm}
                >{\centering\arraybackslash}p{2cm}}
\toprule
\textbf{(Depth, Width)} & \textbf{EM} & \textbf{F1} & \textbf{Time (min)} \\
\midrule
Vanilla / (1,1) & 56.00 & 59.70 & 10 \\
(3,3)           & 63.50 & 65.84 & 40 \\
(3,4)           & 65.00 & 65.69 & 52 \\
(3,5)           & 64.50 & 66.63 & 66 \\
(3,6)           & 65.00 & 64.91 & 83 \\
(4,4)           & 66.50 & 65.36 & 119 \\
(4,5)           & 66.00 & 67.01 & 168 \\
(4,6)           & 67.00 & 66.29 & 266 \\
(5,4)           & 63.50 & 65.52 & 189 \\
(5,5)           & 66.00 & 66.24 & 413 \\
(5,6)           & 65.50 & 65.63 & 770 \\
\bottomrule
\end{tabular}
\caption{\textbf{Computational overhead in relation to the search space.} As the search space expands in depth and width, performance improves but with diminishing returns and significantly increased reasoning time. The (4,5) setting achieves a good trade-off and is adopted in our main experiments.}
\label{tab:search_space_cost}
\end{table}


==> Tables/prompts.tex <==

\begin{table*}[h]
\begin{tabular}{p{14cm}}
\toprule
Your task is to decompose the original question into one smaller sub-question \\ 
based on the Intermediate answer and Observation. \\ 
The decomposed process is encouraged to be done from multiple perspectives. \\ 
Output a thought to reason the original question, \\ 
and output one sub-question that you think is appropriate to solve next. \\ 
DO NOT REPEAT the question and DO NOT try to answer the question. \\ 
The output format is limited to: \\ 
Thought: ... \\ 
Sub-question: ... \\ 
Here, the "..." indicates omitted output information that you need to fill in. \\
\\
Original question: \textcolor{orange}{\{original question\}} \\ 
\\
Intermediate answers: \textcolor{orange}{\{reasoning state\}} \\ 
\\
Observation: \textcolor{orange}{\{retrieved documents\}} \\
\\
Output: \\
\bottomrule
\end{tabular}
\caption{Prompts for Sub-Question Decomposition}
\end{table*}

\vspace{0.5cm} % Adjust space between tables

\begin{table*}[h]
\begin{tabular}{p{14cm}}
\toprule
Your task is to answer the following question using provided supporting facts. \\ 
The output answer should be a complete declarative sentence, \\ 
rather than directly outputting phrases or words. \\ 
Do not use pronouns in the sentence. \\ 
Specially, if no provided supporting facts, \\ 
just output "No directly relevant facts found." and nothing else. \\
\\
Question: \textcolor{orange}{\{sub-question\}}\\
\\
Supporting facts: \textcolor{orange}{\{retrieved documents\}} \\
\\
Output: \\
\bottomrule
\end{tabular}
\caption{Prompts for Intermediate Answer Generation}
\end{table*}

\vspace{0.5cm} % Adjust space between tables

\begin{table*}[h]
\begin{tabular}{p{14cm}}
\toprule
Your task is to answer the original question based on the intermediate answers. \\ 
Output the final answer directly and nothing else. \\
\\
Original question: \textcolor{orange}{\{original question\}} \\
\\
Intermediate answers: \textcolor{orange}{\{reasoning state\}} \\ 
\\
Output: \\
\bottomrule
\end{tabular}
\caption{Prompts for Final Answer Generation}
\end{table*}

\vspace{0.5cm} % Adjust space between tables

\begin{table*}[h]
\begin{tabular}{p{14cm}}
\toprule
Given intermediate answer containing the facts about the original question, \\ 
which is unknown, your task is to infer what the original question might have been. \\ 
Output the most likely original question directly and nothing else. \\
\\
Example 1: \\
Intermediate answer: \\
Muhammad Ali was 74 years old when he died. \\
Alan Turing was 41 years old when he died. \\
The original question might be: \\
Who lived longer, Muhammad Ali or Alan Turing? \\
\\
Example 2: \\
Intermediate answer: \\
Craigslist was founded by Craig Newmark. \\
Craig Newmark was born on December 6, 1952. \\
The original question might be: \\
When was the founder of craigslist born? \\
\\
Intermediate answers: \textcolor{orange}{\{reasoning state\}} \\
The original question might be: \\
\bottomrule
\end{tabular}
\caption{Prompts for Risk-Assessing}
\end{table*}

\vspace{0.5cm} % Adjust space between tables

\begin{table*}[h]
\begin{tabular}{p{14cm}}
\toprule
Given a question, your task is to determine the consistency score of its decomposition sub-questions \\ 
and corresponding intermediate answers with the original question. \\
Directly output JUST A NUMBER between 0 and 10 to represent the consistency score. \\
Do not output anything else. \\
\\
Original question: \textcolor{orange}{\{original question\}} \\
\\
Sub-questions: \textcolor{orange}{\{sub-questions\}} \\
\\
Intermediate answers: \textcolor{orange}{\{reasoning state\}} \\
\\
Output: \\
\bottomrule
\end{tabular}
\caption{Prompts for LLM-as-verifier}
\end{table*}


==> Tables/scale.tex <==
\begin{table*}[t]
\centering
\small % 保持字体大小一致
\renewcommand{\arraystretch}{1.2} % 调整行距
\setlength{\tabcolsep}{3pt} % 调整列间距
\begin{tabular}{c c >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm} 
                >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm} 
                c >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm} 
                >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm} }
\toprule
\multirow{2}{*}{\textbf{Qwen2.5}} & \multicolumn{4}{c}{\textbf{2Wiki}} & \multicolumn{4}{c}{\textbf{Musique}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
                                                    & \textbf{Pass@1} & \textbf{Pass@N} & \textbf{$\Delta$(1-N)} & \textbf{F1}    
                                                    & \textbf{Pass@1} & \textbf{Pass@N} & \textbf{$\Delta$(1-N)} & \textbf{F1}    \\
\midrule
0.5B                                                 & 21.50  & 53.00  & \textbf{31.50}    & 51.80 & 3.50  & 22.00  & \textbf{18.50}    & 52.28 \\
3B                                                   & 36.50  & 50.50  & \textbf{14.00}    & 57.81 & 19.50  & 28.00  & \textbf{8.50}    & 54.78 \\
7B                                                   & 47.50  & 67.00  & \textbf{19.50}    & 61.37 & 29.00  & 52.50  & \textbf{23.50}    & 62.26 \\
14B                                                  & 56.50  & 66.00  & \textbf{9.50}     & 62.61 & 40.50  & 49.00  & \textbf{8.50}     & 65.87 \\
32B                                                  & 60.50  & 66.50  & \textbf{6.00}     & 63.39 & 38.50  & 47.50  & \textbf{8.00}     & 64.04 \\
\bottomrule
\end{tabular}
\caption{Performance vs. model scales. As the model scale increases, the accuracy of the optimal path selection (Pass@1) gradually approaches the upper bound (Pass@N). \sys is able to more effectively utilize the potential of the search space in larger models.}
\label{tab:scale}
\end{table*}

==> src/introduction_old.tex <==
\section{Introduction}

\input{src/introduction_new.tex}

Large Language Models (LLMs) have demonstrated impressive capabilities across a wide range of tasks~\citep{DBLP:journals/corr/abs-2307-10169, DBLP:journals/corr/abs-2303-08774, DBLP:conf/uist/ParkOCMLB23}.
To mitigate their hallucinations, Retrieval-Augmented Generation (RAG) has emerged as a promising technique by accessing external knowledge~\citep{DBLP:journals/corr/abs-2312-10997, DBLP:journals/corr/abs-2309-01219}.
However, even top-tier models integrated with RAG demonstrate considerable limitations in the open-ended, knowledge-intensive, and complex reasoning tasks, which are ubiquitous in high-stakes industries such as science, finance, and healthcare~\citep{DBLP:journals/corr/abs-2406-12753, DBLP:conf/emnlp/WengZX0HLSLZ23, DBLP:journals/corr/abs-2407-12883}.
For example, GPT-4o~\citep{DBLP:journals/corr/abs-2410-21276} achieves less than 20\% accuracy on MusiQue~\citep{DBLP:journals/tacl/TrivediBKS22} for multihop reasoning, even with the assistance of RAG, falling far short of human-level performance~\citep{DBLP:journals/corr/abs-2412-12881}.
\fixme{This performance gap highlights fundamental challenges/urgent needs...}

\begin{figure}[htbp]
\centering
% \includegraphics[width=\linewidth]{Figures/Figure111.png}
\caption{Schematic illustration of error propagation and verification dilemma.
Humans can avoid upstream errors disrupting downstream outcomes by maintaining hypothesis branches and performing effective state assessment. In contrast, LLMs, either due to error propagation in chain reasoning or insufficient validation for path selection, are unable to solve complex problems.
In the diagram, green represents correct retrieval or reasoning, red indicates errors, and yellow denotes invalid steps.
\src{I find the image a bit difficult to understand at least for me.
For example:
1. The instance chosen isn't very well-known. This makes it hard to understand why some LLM-retrieved answers are incorrect. (For instance: the LLM retrieved ``Peter Till was loaned to Villa Park..." Why is the answer ``Peter Till had played for Villa Park" considered wrong?)
2. There are too many elements in the image, making it confusing. (For example: what does the blue dotted line represent? Why does the left side, which shows the LLM reasoning path, also include a human icon?)
3. The image doesn't clearly show why humans don't face the verification dilemma, compared to LLM. It's not apparent from the illustration. In other words, I personally don't feel the image clearly demonstrates the existing flaws in LLMs.}}
\label{Figure 1}
\end{figure}


\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{Figures/pipeline.pdf}
    \caption{pipeline of \texttt{ARise}}
    \vspace{-4mm}
    \label{fig:pipeline}
\end{figure*}



\src{When explaining each research area, perhaps we should list the advantages first, and then the disadvantages, wouldn't that make the structure clearer?}

One line of existing works to this issue follows the ``Iterative RAG'' paradigm \src{Any ref?}, primarily suffers from error propagation~\citep{DBLP:journals/corr/abs-2411-19443, DBLP:conf/acl/ZhaoLJQB23, DBLP:conf/emnlp/PressZMSSL23, DBLP:journals/corr/abs-2312-10997}, where upstream errors can easily yet irreversibly disrupt downstream retrieval or reasoning.
These approaches leverage iterative retrieval to generate more fine-grained and authentic reasoning steps within the chain-of-thought (CoT) \citep{DBLP:conf/nips/Wei0SBIXCLZ22}.
Conversely, dense reasoning better harnesses the potential of RAG.
Nonetheless, retrieval and generation under this paradigm still proceed sequentially in a left-to-right fashion.
This inevitably results in step-by-step propagation of errors, as illustrated in Figure \ref{Figure 1}.
\src{The \emph{Iterative RAG} paradigm improves reasoning by repeatedly retrieving information, leading to more refined and appropriate steps in the chain-of-thought (CoT) \citep{DBLP:conf/nips/Wei0SBIXCLZ22}. However, it is prone to error propagation~\citep{DBLP:journals/corr/abs-2411-19443, DBLP:conf/acl/ZhaoLJQB23, DBLP:conf/emnlp/PressZMSSL23, DBLP:journals/corr/abs-2312-10997}. Because retrieval and generation in this paradigm still proceed in a left-to-right sequence, upstream errors can easily and irreversibly compromise downstream retrieval or reasoning, leading to a cascade of errors.}


Another line explores the ``Search-based RAG'' paradigm, where the bottleneck lies in the issue of verification for selecting the optimal candidate solutions \citep{DBLP:conf/iclr/LightmanKBEBLLS24, DBLP:journals/corr/abs-2402-06457}.
The core idea behind these approaches is to maintain multiple hypothesis branches through search algorithms such as Monte Carlo Tree Search (MCTS), rather than leaning solely on the top-1 result.
Verification in prior works largely depend on (1) majority voting \citep{DBLP:conf/iclr/0002WSLCNCZ23, feng2025airrag} or (2) fine-tuned LLMs, commonly referred to as reward models, being verifiers \citep{DBLP:journals/corr/abs-2412-12881, DBLP:conf/nips/YaoYZS00N23}.
The former leads to redundant rollouts \src{Any ref?},
while the latter is unscalable due to the difficulty in obtaining reliable training resources \citep{DBLP:journals/corr/abs-2410-08146, deepseek-r1}, particular on knowledge-intensive tasks that involve various topics and dynamic retrieval.
\src{Another approach is the \emph{Search-based RAG} paradigm, which maintains multiple hypothesis branches using search algorithms like Monte Carlo Tree Search (MCTS), rather than relying solely on the top-1 retrieved result. This paradigm primarily depends on either (1) majority voting \citep{DBLP:conf/iclr/0002WSLCNCZ23, feng2025airrag} or (2) fine-tuned LLMs as verifiers \citep{DBLP:journals/corr/abs-2412-12881, DBLP:conf/nips/YaoYZS00N23}. However, the former suffers from redundant rollouts, making it difficult to select the optimal solution. The latter faces challenges in acquiring reliable training data, particularly for knowledge-intensive tasks involving diverse topics and dynamic retrieval \citep{DBLP:journals/corr/abs-2410-08146, deepseek-r1}.}


To address the aforementioned limitations, we propose \texttt{ARise} in this paper.
In general, the MCTS algorithm maintains multiple reasoning trajectories, while the Risk-Value framework computes node values to guide the search process.
Specifically, LLMs generate a complete reasoning trajectory by interleaving problem decomposition and retrieval-generation steps, enabling more precise, granular and intensive reasoning, which facilitates retrieval in turn.
The tree structure promotes exploration of new avenues, and flexible decision-making at branching points mitigate error propagation, allowing LLMs to dynamically create, optimize, and adjust high-level acting plans.
Finally, we design the Risk-Value framework to conduct risk assessment of intermediate reasoning state under Bayesian principles.
This framework provides direct, effective, and training-free verification for the tree search process.

We conducted extensive experiments with multiple LLMs on three open-ended, knowledge-intensive, complex reasoning benchmarks: HotpotQA \citep{DBLP:conf/emnlp/Yang0ZBCSM18}, 2WikiMultihopQA \citep{DBLP:conf/coling/HoNSA20}, and MusiQue \citep{DBLP:journals/tacl/TrivediBKS22}.
These tasks cover a wide range of topics without being constrained by any existing knowledge base or schema.
We show that \texttt{ARise} obtains superior results through a diversified decision-making process and reliable path selection, outperforming the advanced baselines across the board.
We also demonstrate the effectiveness of the Risk-Value framework with ablation studies and further analyze how model size and inference spend affects performance.

To summarize, our contributions are as follows:
%\wk{The first contribution is a brief introduction of \texttt{ARise}, like its designs and novitiates. The second contribution emphasizes issues it can address and the excellent results. The third could be the inspiration and other outcomes from deep analysis or observations.}
\begin{itemize}
\item We propose \texttt{ARise} that overcomes two major bottlenecks in existing reasoning-based RAG approaches, namely error propagation and verification dilemma.

\item We conduct extensive experiments on open-ended, knowledge-intensive, and complex reasoning tasks, showing that \texttt{ARise} achieves state-of-the-art performance.

\item We design a direct, efficient, and generalizable verification method that moves away from the current redundant majority voting and unscalable post-training paradigms.
\end{itemize}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../main"
%%% End:

